The interplay between forming planets and photo-evaporating discs I: Forbidden line diagnostics

Disc winds and planet formation are considered to be two of the most important mechanisms that drive the evolution and dispersal of protoplanetary discs and in turn define the environment in which planets form and evolve. While both have been studied extensively in the past, we combine them into one model by performing three-dimensional radiation-hydrodynamic simulations of giant planet hosting discs that are undergoing X-ray photo-evaporation, with the goal to analyse the interactions between both mechanisms. In order to study the effect on observational diagnostics, we produce synthetic observations of commonly used wind-tracing forbidden emission lines with detailed radiative transfer and photo-ionisation calculations. We find that a sufficiently massive giant planet carves a gap in the gas disc that is deep enough to affect the structure and kinematics of the pressure-driven photo-evaporative wind significantly. This effect can be strong enough to be visible in the synthetic high-resolution observations of some of our wind diagnostic lines, such as the [OI] 6300 \r{A} or [SII] 6730 \r{A} lines. When the disc is observed at inclinations around 40{\deg} and higher, the spectral line profiles may exhibit a peak in the redshifted part of the spectrum, which cannot easily be explained by simple wind models alone. Moreover, massive planets can induce asymmetric substructures within the disc and the photo-evaporative wind, giving rise to temporal variations of the line profiles that can be strong enough to be observable on timescales of less than a quarter of the planet's orbital period.

==> 4-discussion.tex <==
% combined with results

==> tables/fits_feii-17_1.tex <==
\begin{tabular}{ll|llll|llll|llll}
      &     & \multicolumn{4}{c}{MJ1} & \multicolumn{4}{c}{MJ5} & \multicolumn{4}{c}{REF} \\
    i[\degree] & phi [\degree] & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$)  \\
    \hline
    \hline
    0 & 0 & -3.41 & -3.38 & 9.75 & -5.27  & -3.77 & -3.88 & 9.42 & -5.44  & -3.37 & -3.13 & 9.42 & -4.97  \\
    \hline
    20 & 0 & -3.41 & -3.63 & 11.34 & -5.27  & -3.28 & -3.38 & 10.94 & -5.45  & -3.37 & -3.38 & 10.70 & -4.98  \\
     & 25 & -3.44 & -3.63 & 11.33 & -5.27  & -3.28 & -3.38 & 10.89 & -5.45  & & & &  \\
     & 50 & -3.46 & -3.63 & 11.37 & -5.27  & -3.35 & -3.38 & 11.04 & -5.44  & & & &  \\
     & 75 & -3.49 & -3.63 & 11.44 & -5.27  & -3.48 & -3.63 & 11.29 & -5.44  & & & &  \\
     & 100 & -3.51 & -3.88 & 11.50 & -5.27  & -3.62 & -3.88 & 11.44 & -5.44  & & & &  \\
     & 125 & -3.52 & -3.88 & 11.55 & -5.27  & -3.76 & -3.88 & 11.41 & -5.44  & & & &  \\
     & 150 & -3.50 & -3.63 & 11.58 & -5.27  & -3.89 & -4.14 & 11.21 & -5.45  & & & &  \\
     & 175 & -3.47 & -3.63 & 11.58 & -5.27  & -3.97 & -4.39 & 10.92 & -5.45  & & & &  \\
     & 200 & -3.43 & -3.63 & 11.50 & -5.27  & -3.94 & -4.14 & 10.74 & -5.45  & & & &  \\
     & 225 & -3.40 & -3.38 & 11.37 & -5.27  & -3.83 & -3.88 & 10.77 & -5.45  & & & &  \\
     & 250 & -3.36 & -3.38 & 11.28 & -5.27  & -3.70 & -3.63 & 10.97 & -5.45  & & & &  \\
     & 275 & -3.33 & -3.38 & 11.27 & -5.27  & -3.58 & -3.63 & 11.25 & -5.45  & & & &  \\
     & 300 & -3.34 & -3.38 & 11.29 & -5.27  & -3.49 & -3.63 & 11.37 & -5.45  & & & &  \\
     & 325 & -3.37 & -3.38 & 11.33 & -5.27  & -3.39 & -3.38 & 11.24 & -5.45  & & & &  \\
     & 350 & -3.40 & -3.63 & 11.34 & -5.27  & -3.30 & -3.38 & 11.01 & -5.45  & & & & 
\end{tabular}

==> tables/fits_feii-17_2.tex <==
\begin{tabular}{ll|llll|llll|llll}
      &     & \multicolumn{4}{c}{MJ1} & \multicolumn{4}{c}{MJ5} & \multicolumn{4}{c}{REF} \\
    i[°] & phi [°] & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$)  \\
    \hline
    \hline
    40 & 0 & -2.95 & -4.14 & 15.78 & -5.27  & -2.18 & -1.13 & 14.82 & -5.44  & -2.86 & -3.38 & 15.00 & -4.98  \\
     & 25 & -2.94 & -3.88 & 15.81 & -5.28  & -2.19 & -1.38 & 14.50 & -5.44  & & & &  \\
     & 50 & -2.94 & -3.88 & 16.06 & -5.28  & -2.44 & -2.38 & 15.06 & -5.45  & & & &  \\
     & 75 & -2.99 & -4.39 & 16.19 & -5.27  & -2.73 & -3.38 & 15.84 & -5.45  & & & &  \\
     & 100 & -3.06 & -4.64 & 16.10 & -5.27  & -2.98 & -2.88 & 16.68 & -5.45  & & & &  \\
     & 125 & -3.07 & -4.39 & 16.09 & -5.27  & -3.22 & -1.88 & 16.98 & -5.45  & & & &  \\
     & 150 & -3.01 & -3.88 & 16.21 & -5.28  & -3.48 & -4.64 & 16.34 & -5.45  & & & &  \\
     & 175 & -2.95 & -3.63 & 16.28 & -5.28  & -3.68 & -4.64 & 14.85 & -5.44  & & & &  \\
     & 200 & -2.91 & -3.63 & 16.17 & -5.28  & -3.63 & -4.14 & 14.18 & -5.45  & & & &  \\
     & 225 & -2.87 & -3.13 & 15.96 & -5.28  & -3.35 & -3.13 & 14.53 & -5.45  & & & &  \\
     & 250 & -2.81 & -2.88 & 15.88 & -5.28  & -3.03 & -1.63 & 15.09 & -5.45  & & & &  \\
     & 275 & -2.76 & -2.88 & 15.94 & -5.28  & -2.83 & -1.13 & 16.04 & -5.45  & & & &  \\
     & 300 & -2.78 & -3.13 & 15.93 & -5.27  & -2.67 & -0.63 & 16.92 & -5.45  & & & &  \\
     & 325 & -2.86 & -3.63 & 15.94 & -5.27  & -2.47 & -0.88 & 16.58 & -5.45  & & & &  \\
     & 350 & -2.93 & -4.14 & 15.83 & -5.27  & -2.24 & -1.13 & 15.28 & -5.44  & & & &  \\
    \hline
    60 & 0 & -1.94 & -5.89 & 19.96 & -5.27  & -0.75 & 2.13 & 18.36 & -5.44  & -1.85 & -6.14 & 19.22 & -4.98  \\
     & 25 & -1.91 & -6.39 & 20.16 & -5.28  & -0.79 & 1.63 & 17.84 & -5.44  & & & &  \\
     & 50 & -1.90 & -6.64 & 20.45 & -5.28  & -1.19 & 0.63 & 19.01 & -5.45  & & & &  \\
     & 75 & -1.99 & -6.64 & 20.41 & -5.27  & -1.63 & -4.39 & 19.94 & -5.45  & & & &  \\
     & 100 & -2.11 & -6.64 & 20.15 & -5.27  & -1.96 & -5.89 & 21.20 & -5.45  & & & &  \\
     & 125 & -2.10 & -6.39 & 20.31 & -5.27  & -2.25 & 2.63 & 21.55 & -5.44  & & & &  \\
     & 150 & -2.00 & -6.39 & 20.67 & -5.28  & -2.61 & -7.64 & 20.57 & -5.44  & & & &  \\
     & 175 & -1.91 & 2.13 & 20.64 & -5.28  & -2.93 & -5.89 & 18.71 & -5.44  & & & &  \\
     & 200 & -1.89 & -6.39 & 20.58 & -5.28  & -2.92 & -4.89 & 17.56 & -5.45  & & & &  \\
     & 225 & -1.86 & -6.14 & 20.48 & -5.28  & -2.52 & -4.89 & 18.45 & -5.45  & & & &  \\
     & 250 & -1.78 & 2.38 & 20.53 & -5.28  & -2.05 & 1.13 & 19.11 & -5.44  & & & &  \\
     & 275 & -1.69 & 2.38 & 20.47 & -5.27  & -1.75 & 2.13 & 20.38 & -5.44  & & & &  \\
     & 300 & -1.70 & 2.13 & 20.59 & -5.28  & -1.53 & 3.88 & 21.38 & -5.44  & & & &  \\
     & 325 & -1.81 & -5.89 & 20.54 & -5.28  & -1.23 & 3.88 & 20.88 & -5.44  & & & &  \\
     & 350 & -1.92 & -5.89 & 20.01 & -5.27  & -0.87 & 2.63 & 19.15 & -5.44  & & & &  \\
    \hline
    80 & 0 & -0.61 & -5.89 & 22.10 & -5.27  & 0.74 & 4.64 & 20.30 & -5.44  & 5.20 & -6.14 & 10.98 & -5.28  \\
     &  & & & &  & & & &  & -6.51 & -6.14 & 10.62 & -5.30  \\
     & 25 & -0.59 & -6.39 & 22.27 & -5.27  & 0.69 & 4.39 & 19.54 & -5.44  & & & &  \\
     & 50 & 5.37 & -6.39 & 12.10 & -5.56  & 0.19 & 4.14 & 20.96 & -5.45  & & & &  \\
     &  & -7.03 & -6.39 & 11.15 & -5.60  & & & &  & & & &  \\
     & 75 & 5.51 & -6.64 & 12.42 & -5.56  & -0.34 & -4.39 & 21.94 & -5.44  & & & &  \\
     &  & -7.06 & -6.64 & 11.04 & -5.60  & & & &  & & & &  \\
     & 100 & 5.61 & -6.39 & 12.73 & -5.57  & 6.15 & -5.64 & 12.02 & -5.78  & & & &  \\
     &  & -6.99 & -6.39 & 11.03 & -5.59  & -6.65 & -5.64 & 12.79 & -5.72  & & & &  \\
     & 125 & -0.82 & -6.14 & 22.47 & -5.27  & 5.33 & -7.89 & 12.26 & -5.73  & & & &  \\
     &  & & & &  & -8.04 & -7.89 & 11.09 & -5.78  & & & &  \\
     & 150 & -0.68 & -6.64 & 22.84 & -5.27  & 4.76 & -7.64 & 12.68 & -5.72  & & & &  \\
     &  & & & &  & -8.08 & -7.64 & 10.44 & -5.79  & & & &  \\
     & 175 & -0.58 & 4.64 & 22.38 & -5.27  & -1.82 & -6.14 & 20.68 & -5.44  & & & &  \\
     & 200 & -0.47 & 5.14 & 21.79 & -6.02  & -1.85 & -5.14 & 19.42 & -5.44  & & & &  \\
     &  & -0.59 & 5.14 & 21.79 & -5.34  & & & &  & & & &  \\
     & 225 & 5.64 & -6.14 & 11.65 & -5.58  & -1.39 & -5.39 & 20.41 & -5.45  & & & &  \\
     &  & -6.73 & -6.14 & 11.65 & -5.58  & & & &  & & & &  \\
     & 250 & 5.63 & 5.39 & 10.77 & -5.66  & -0.84 & 3.13 & 21.52 & -5.44  & & & &  \\
     &  & 0.32 & 5.39 & 28.78 & -6.06  & & & &  & & & &  \\
     &  & -6.70 & 5.39 & 11.30 & -5.64  & & & &  & & & &  \\
     & 275 & 5.69 & 5.14 & 11.45 & -5.58  & -0.47 & 4.14 & 22.89 & -5.44  & & & &  \\
     &  & -6.90 & 5.14 & 12.13 & -5.59  & & & &  & & & &  \\
     & 300 & -0.34 & 4.89 & 22.55 & -5.27  & 7.45 & -6.64 & 9.42 & -6.07  & & & &  \\
     &  & & & &  & -0.53 & -6.64 & 20.45 & -5.71  & & & &  \\
     &  & & & &  & -7.67 & -6.64 & 9.42 & -6.10  & & & &  \\
     & 325 & -0.47 & -5.89 & 22.89 & -5.27  & 6.83 & 6.64 & 10.77 & -5.77  & & & &  \\
     &  & & & &  & -6.24 & 6.64 & 11.96 & -5.74  & & & &  \\
     & 350 & -0.59 & -5.89 & 22.16 & -5.27  & 0.61 & 5.39 & 21.10 & -5.44  & & & & 
\end{tabular}

==> tables/fits_neii-12_1.tex <==
\begin{tabular}{ll|llll|llll|llll}
      &     & \multicolumn{4}{c}{MJ1} & \multicolumn{4}{c}{MJ5} & \multicolumn{4}{c}{REF} \\
    i[\degree] & phi [\degree] & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$)  \\
    \hline
    \hline
    0 & 0 & -2.84 & -2.88 & 11.32 & -5.61  & -2.25 & -2.38 & 11.50 & -5.68  & -2.57 & -2.13 & 10.60 & -5.57  \\
    \hline
    20 & 0 & -3.15 & -3.88 & 13.63 & -5.61  & -2.00 & -2.13 & 13.16 & -5.69  & -3.10 & -3.88 & 13.25 & -5.57  \\
     & 25 & -3.16 & -3.88 & 13.62 & -5.61  & -1.98 & -2.38 & 13.47 & -5.68  & & & &  \\
     & 50 & -3.17 & -4.14 & 13.83 & -5.61  & -2.02 & -2.38 & 13.88 & -5.68  & & & &  \\
     & 75 & -3.19 & -4.14 & 14.18 & -5.61  & -2.13 & -2.63 & 14.33 & -5.68  & & & &  \\
     & 100 & -3.24 & -4.39 & 14.43 & -5.61  & -2.27 & -2.88 & 14.61 & -5.68  & & & &  \\
     & 125 & -3.31 & -4.39 & 14.46 & -5.61  & -2.41 & -3.38 & 14.71 & -5.68  & & & &  \\
     & 150 & -3.38 & -4.39 & 14.23 & -5.62  & -2.53 & -3.63 & 14.66 & -5.68  & & & &  \\
     & 175 & -3.43 & -4.14 & 13.82 & -5.62  & -2.64 & -3.63 & 14.37 & -5.68  & & & &  \\
     & 200 & -3.41 & -4.14 & 13.43 & -5.62  & -2.68 & -3.63 & 13.89 & -5.68  & & & &  \\
     & 225 & -3.32 & -3.88 & 13.21 & -5.62  & -2.64 & -3.13 & 13.32 & -5.69  & & & &  \\
     & 250 & -3.21 & -3.63 & 13.21 & -5.62  & -2.50 & -2.63 & 12.90 & -5.69  & & & &  \\
     & 275 & -3.13 & -3.63 & 13.37 & -5.61  & -2.35 & -2.38 & 12.74 & -5.69  & & & &  \\
     & 300 & -3.11 & -3.88 & 13.55 & -5.61  & -2.22 & -2.13 & 12.75 & -5.69  & & & &  \\
     & 325 & -3.12 & -3.88 & 13.66 & -5.61  & -2.11 & -2.13 & 12.87 & -5.69  & & & &  \\
     & 350 & -3.14 & -3.88 & 13.65 & -5.61  & -2.02 & -2.13 & 13.06 & -5.69  & & & &  \\
    \hline
    40 & 0 & -2.99 & -5.39 & 19.40 & -5.61  & -1.21 & -0.13 & 18.06 & -5.69  & -2.89 & -5.39 & 19.20 & -5.57  \\
     & 25 & -2.92 & -4.64 & 19.37 & -5.62  & -1.16 & -0.38 & 18.02 & -5.68  & & & &  \\
     & 50 & -2.79 & -4.14 & 20.06 & -5.62  & -1.33 & -0.88 & 18.64 & -5.68  & & & &  \\
     & 75 & -2.74 & -5.39 & 20.65 & -5.62  & -1.66 & -1.88 & 19.56 & -5.69  & & & &  \\
     & 100 & -2.84 & -5.64 & 20.68 & -5.61  & -1.98 & -3.13 & 20.34 & -5.69  & & & &  \\
     & 125 & -2.96 & -5.39 & 20.59 & -5.61  & -2.21 & -2.38 & 20.96 & -5.69  & & & &  \\
     & 150 & -3.06 & -5.39 & 20.38 & -5.62  & -2.40 & -3.13 & 20.87 & -5.69  & & & &  \\
     & 175 & -3.16 & -5.39 & 19.83 & -5.62  & -2.63 & -4.14 & 19.55 & -5.68  & & & &  \\
     & 200 & -3.17 & -5.14 & 19.24 & -5.62  & -2.78 & -3.88 & 17.98 & -5.69  & & & &  \\
     & 225 & -3.09 & -4.14 & 18.87 & -5.62  & -2.65 & -3.13 & 16.75 & -5.70  & & & &  \\
     & 250 & -2.95 & -3.63 & 19.01 & -5.62  & -2.26 & -1.88 & 16.32 & -5.70  & & & &  \\
     & 275 & -2.86 & -4.39 & 19.48 & -5.62  & -1.89 & -0.88 & 16.67 & -5.69  & & & &  \\
     & 300 & -2.90 & -4.89 & 19.69 & -5.61  & -1.66 & -0.63 & 17.36 & -5.69  & & & &  \\
     & 325 & -2.97 & -5.39 & 19.71 & -5.61  & -1.47 & 0.13 & 17.89 & -5.69  & & & &  \\
     & 350 & -3.00 & -5.39 & 19.52 & -5.61  & -1.27 & 0.13 & 18.10 & -5.69  & & & & 
\end{tabular}

==> tables/fits_neii-12_2.tex <==
\begin{tabular}{ll|llll|llll|llll}
      &     & \multicolumn{4}{c}{MJ1} & \multicolumn{4}{c}{MJ5} & \multicolumn{4}{c}{REF} \\
    i[°] & phi [°] & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$)  \\
    \hline
    \hline
    60 & 0 & -2.00 & -6.89 & 25.11 & -5.61  & -0.15 & 3.63 & 22.46 & -5.68  & -1.93 & -7.64 & 24.62 & -5.57  \\
     & 25 & -1.89 & -7.14 & 25.03 & -5.62  & -0.01 & 2.38 & 21.95 & -5.69  & & & &  \\
     & 50 & -1.73 & 2.88 & 25.42 & -5.62  & -0.27 & 1.63 & 22.24 & -5.68  & & & &  \\
     & 75 & -1.68 & -7.39 & 25.93 & -5.61  & -0.83 & -2.88 & 23.91 & -5.69  & & & &  \\
     & 100 & -1.80 & -7.39 & 25.98 & -5.61  & -1.32 & -5.64 & 24.72 & -5.68  & & & &  \\
     & 125 & -1.91 & -7.14 & 26.30 & -5.61  & -1.61 & -7.64 & 25.60 & -5.68  & & & &  \\
     & 150 & -1.99 & -7.14 & 26.34 & -5.62  & -1.86 & -7.64 & 25.59 & -5.69  & & & &  \\
     & 175 & -2.10 & -7.39 & 25.65 & -5.62  & -2.21 & -5.39 & 23.89 & -5.68  & & & &  \\
     & 200 & -2.16 & -7.14 & 24.85 & -5.62  & -2.50 & -4.39 & 21.73 & -5.69  & & & &  \\
     & 225 & -2.14 & -6.89 & 24.49 & -5.62  & -2.34 & -4.14 & 20.41 & -5.70  & & & &  \\
     & 250 & -2.05 & -7.14 & 24.84 & -5.62  & -1.73 & -0.88 & 20.93 & -5.70  & & & &  \\
     & 275 & -1.96 & -7.64 & 25.63 & -5.62  & -1.18 & 2.13 & 21.90 & -5.69  & & & &  \\
     & 300 & -1.96 & -7.14 & 26.32 & -5.62  & -0.88 & 3.63 & 23.04 & -5.69  & & & &  \\
     & 325 & -2.01 & -6.89 & 26.02 & -5.61  & -0.62 & 4.14 & 23.19 & -5.68  & & & &  \\
     & 350 & -2.02 & -6.89 & 25.30 & -5.61  & -0.28 & 3.88 & 22.67 & -5.68  & & & &  \\
    \hline
    80 & 0 & -0.59 & -6.64 & 28.29 & -5.61  & 0.91 & 5.39 & 25.21 & -5.68  & -0.60 & -7.39 & 27.58 & -5.57  \\
     & 25 & -0.49 & -6.89 & 28.05 & -5.62  & 1.15 & 4.39 & 23.93 & -5.69  & & & &  \\
     & 50 & -0.36 & 5.64 & 27.57 & -5.61  & 0.84 & 4.14 & 23.76 & -5.69  & & & &  \\
     & 75 & -0.35 & -7.14 & 28.35 & -5.61  & 0.13 & -3.63 & 25.61 & -5.69  & & & &  \\
     & 100 & -0.46 & -7.14 & 28.59 & -5.60  & -0.46 & -5.89 & 26.25 & -5.68  & & & &  \\
     & 125 & -0.53 & -6.89 & 29.40 & -5.61  & 6.41 & -7.64 & 15.19 & -5.97  & & & &  \\
     &  & & & &  & -8.65 & -7.64 & 13.34 & -6.03  & & & &  \\
     & 150 & -0.58 & -6.64 & 29.68 & -5.62  & 6.26 & -7.89 & 15.41 & -5.98  & & & &  \\
     &  & & & &  & -8.78 & -7.89 & 13.62 & -6.02  & & & &  \\
     & 175 & -0.68 & -6.89 & 28.86 & -5.62  & -1.51 & -6.14 & 25.83 & -5.68  & & & &  \\
     & 200 & -0.77 & -6.89 & 27.85 & -5.61  & -1.85 & -4.64 & 23.99 & -5.69  & & & &  \\
     & 225 & -0.84 & -6.89 & 27.20 & -5.61  & -1.67 & -4.89 & 23.01 & -5.69  & & & &  \\
     & 250 & -0.81 & -7.39 & 27.75 & -5.61  & -0.95 & -4.89 & 24.57 & -5.70  & & & &  \\
     & 275 & -0.72 & 5.64 & 28.45 & -5.61  & -0.32 & 4.64 & 25.15 & -5.68  & & & &  \\
     & 300 & -0.67 & 5.39 & 29.50 & -5.61  & 7.16 & 6.39 & 13.61 & -6.00  & & & &  \\
     &  & & & &  & -7.31 & 6.39 & 14.17 & -6.00  & & & &  \\
     & 325 & -0.67 & -6.14 & 29.56 & -5.62  & 7.42 & 6.64 & 13.69 & -6.00  & & & &  \\
     &  & & & &  & -7.26 & 6.64 & 14.02 & -6.01  & & & &  \\
     & 350 & -0.62 & -6.39 & 28.51 & -5.61  & 0.74 & 5.89 & 25.69 & -5.68  & & & & 
\end{tabular}

==> tables/fits_sii-4068_1.tex <==
\begin{tabular}{ll|llll|llll|llll}
      &     & \multicolumn{4}{c}{MJ1} & \multicolumn{4}{c}{MJ5} & \multicolumn{4}{c}{REF} \\
    i[\degree] & phi [\degree] & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$)  \\
    \hline
    \hline
    0 & 0 & -0.61 & -0.63 & 9.59 & -5.06  & -0.90 & -0.63 & 10.77 & -4.79  & -0.90 & -0.63 & 9.42 & -4.83  \\
    \hline
    20 & 0 & -0.73 & -2.13 & 16.78 & -5.05  & -1.29 & -1.88 & 15.61 & -4.79  & -1.59 & -3.63 & 16.61 & -4.83  \\
     & 25 & -0.80 & -2.38 & 16.86 & -5.05  & -1.16 & -1.88 & 15.71 & -4.78  & & & &  \\
     & 50 & -0.82 & -3.13 & 17.23 & -5.05  & -1.05 & -1.63 & 16.05 & -4.78  & & & &  \\
     & 75 & -0.77 & -3.63 & 17.91 & -5.05  & -1.00 & -1.63 & 16.43 & -4.79  & & & &  \\
     & 100 & -0.71 & -3.88 & 18.72 & -5.05  & -1.02 & -1.88 & 16.67 & -4.79  & & & &  \\
     & 125 & -0.74 & -4.14 & 19.33 & -5.05  & -1.07 & -2.38 & 16.90 & -4.78  & & & &  \\
     & 150 & -0.87 & -4.14 & 19.51 & -5.05  & -1.09 & -2.88 & 17.44 & -4.79  & & & &  \\
     & 175 & -1.08 & -4.39 & 19.10 & -5.05  & -1.12 & -3.63 & 18.00 & -4.79  & & & &  \\
     & 200 & -1.29 & -3.88 & 18.17 & -5.04  & -1.18 & -3.63 & 18.07 & -4.78  & & & &  \\
     & 225 & -1.38 & -3.38 & 17.17 & -5.05  & -1.27 & -3.13 & 17.73 & -4.78  & & & &  \\
     & 250 & -1.29 & -2.88 & 16.51 & -5.05  & -1.36 & -2.38 & 17.20 & -4.78  & & & &  \\
     & 275 & -1.10 & -2.13 & 16.21 & -5.05  & -1.44 & -2.13 & 16.71 & -4.78  & & & &  \\
     & 300 & -0.90 & -1.88 & 16.30 & -5.05  & -1.49 & -2.13 & 16.22 & -4.79  & & & &  \\
     & 325 & -0.75 & -1.88 & 16.60 & -5.05  & -1.46 & -1.88 & 15.83 & -4.79  & & & &  \\
     & 350 & -0.72 & -1.88 & 16.76 & -5.05  & -1.35 & -1.88 & 15.64 & -4.79  & & & &  \\
    \hline
    40 & 0 & 6.58 & -8.65 & 18.19 & -5.29  & -1.00 & 2.13 & 25.36 & -4.79  & -1.56 & -7.64 & 27.56 & -4.83  \\
     &  & -9.41 & -8.65 & 13.63 & -5.42  & & & &  & & & &  \\
     & 25 & 5.93 & -8.65 & 19.63 & -5.26  & -0.87 & 0.88 & 25.59 & -4.79  & & & &  \\
     &  & -9.75 & -8.65 & 13.39 & -5.46  & & & &  & & & &  \\
     & 50 & 4.56 & -9.15 & 21.45 & -5.20  & -0.85 & 0.88 & 25.94 & -4.79  & & & &  \\
     &  & -10.68 & -9.15 & 11.75 & -5.57  & & & &  & & & &  \\
     & 75 & 5.32 & -9.40 & 20.13 & -5.23  & -0.93 & -2.38 & 26.59 & -4.79  & & & &  \\
     &  & -10.61 & -9.40 & 12.31 & -5.52  & & & &  & & & &  \\
     & 100 & 7.08 & -9.15 & 17.93 & -5.29  & -1.05 & -6.39 & 26.78 & -4.79  & & & &  \\
     &  & -9.79 & -9.15 & 14.27 & -5.41  & & & &  & & & &  \\
     & 125 & 8.49 & -8.90 & 16.91 & -5.35  & -1.12 & -7.64 & 27.16 & -4.79  & & & &  \\
     &  & -9.08 & -8.90 & 15.94 & -5.35  & & & &  & & & &  \\
     & 150 & 8.28 & -9.15 & 18.30 & -5.33  & 2.99 & -8.65 & 21.63 & -4.91  & & & &  \\
     &  & -9.52 & -9.15 & 15.73 & -5.36  & -10.66 & -8.65 & 11.03 & -5.39  & & & &  \\
     & 175 & 7.38 & -9.15 & 20.12 & -5.30  & 3.88 & -7.39 & 20.89 & -4.95  & & & &  \\
     &  & -10.05 & -9.15 & 14.79 & -5.40  & -10.27 & -7.39 & 12.44 & -5.29  & & & &  \\
     & 200 & 6.39 & -8.65 & 21.47 & -5.28  & -1.24 & -4.64 & 27.04 & -4.78  & & & &  \\
     &  & -10.08 & -8.65 & 14.39 & -5.44  & & & &  & & & &  \\
     & 225 & -1.47 & -8.15 & 28.87 & -5.04  & -1.30 & -3.13 & 26.37 & -4.78  & & & &  \\
     & 250 & -1.38 & -7.64 & 28.14 & -5.05  & -1.28 & -1.63 & 25.76 & -4.78  & & & &  \\
     & 275 & -1.19 & -7.39 & 27.74 & -5.05  & -1.27 & -0.63 & 25.35 & -4.78  & & & &  \\
     & 300 & -0.97 & -7.64 & 27.92 & -5.04  & -1.29 & -0.38 & 25.05 & -4.78  & & & &  \\
     & 325 & 6.57 & -8.15 & 17.69 & -5.30  & -1.24 & 0.63 & 24.82 & -4.79  & & & &  \\
     &  & -9.27 & -8.15 & 13.71 & -5.41  & & & &  & & & &  \\
     & 350 & 6.69 & -8.65 & 17.82 & -5.30  & -1.07 & 2.13 & 25.13 & -4.79  & & & &  \\
     &  & -9.35 & -8.65 & 13.65 & -5.42  & & & &  & & & & 
\end{tabular}

==> tables/fits_sii-4068_2.tex <==
\begin{tabular}{ll|llll|llll|llll}
      &     & \multicolumn{4}{c}{MJ1} & \multicolumn{4}{c}{MJ5} & \multicolumn{4}{c}{REF} \\
    i[°] & phi [°] & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$)  \\
    \hline
    \hline
    60 & 0 & 9.57 & -11.90 & 22.57 & -5.30  & -0.48 & 5.89 & 32.42 & -4.78  & -1.02 & -9.65 & 36.26 & -4.83  \\
     &  & -12.35 & -11.90 & 17.59 & -5.41  & & & &  & & & &  \\
     & 25 & 9.30 & -11.15 & 23.30 & -5.29  & -0.34 & 4.89 & 32.71 & -4.78  & & & &  \\
     &  & -12.32 & -11.15 & 17.94 & -5.42  & & & &  & & & &  \\
     & 50 & 8.04 & -11.65 & 24.79 & -5.25  & -0.38 & 3.88 & 33.02 & -4.78  & & & &  \\
     &  & -13.08 & -11.65 & 16.52 & -5.49  & & & &  & & & &  \\
     & 75 & 8.34 & 8.15 & 23.56 & -5.26  & -0.55 & 4.14 & 34.59 & -4.79  & & & &  \\
     &  & -12.93 & 8.15 & 16.76 & -5.47  & & & &  & & & &  \\
     & 100 & 10.16 & 10.65 & 20.85 & -5.32  & 7.05 & -7.39 & 22.88 & -5.01  & & & &  \\
     &  & -11.79 & 10.65 & 18.98 & -5.38  & -11.18 & -7.39 & 16.82 & -5.19  & & & &  \\
     & 125 & 12.61 & -10.90 & 17.92 & -5.41  & 6.19 & -9.65 & 24.19 & -4.97  & & & &  \\
     &  & 1.32 & -10.90 & 9.42 & -6.37  & -12.10 & -9.65 & 15.22 & -5.26  & & & &  \\
     &  & -11.24 & -10.90 & 20.07 & -5.34  & & & &  & & & &  \\
     & 150 & 11.48 & -11.65 & 21.58 & -5.35  & 5.46 & -10.15 & 25.17 & -4.95  & & & &  \\
     &  & -11.68 & -11.65 & 20.25 & -5.35  & -12.80 & -10.15 & 14.49 & -5.31  & & & &  \\
     & 175 & 10.55 & -11.65 & 23.53 & -5.32  & 7.02 & -8.40 & 23.74 & -5.00  & & & &  \\
     &  & -12.41 & -11.65 & 19.02 & -5.38  & -11.61 & -8.40 & 16.96 & -5.20  & & & &  \\
     & 200 & 9.79 & -11.15 & 24.52 & -5.31  & -1.00 & -5.14 & 33.86 & -4.78  & & & &  \\
     &  & -12.41 & -11.15 & 18.75 & -5.40  & & & &  & & & &  \\
     & 225 & 9.09 & -10.65 & 24.52 & -5.31  & -1.02 & -4.64 & 33.38 & -4.78  & & & &  \\
     &  & -12.14 & -10.65 & 18.81 & -5.40  & & & &  & & & &  \\
     & 250 & 8.43 & -9.90 & 24.12 & -5.30  & -0.89 & -4.14 & 33.13 & -4.78  & & & &  \\
     &  & -11.95 & -9.90 & 18.40 & -5.41  & & & &  & & & &  \\
     & 275 & 8.27 & -10.40 & 23.78 & -5.29  & -0.78 & 4.14 & 33.44 & -4.79  & & & &  \\
     &  & -11.97 & -10.40 & 17.62 & -5.43  & & & &  & & & &  \\
     & 300 & 8.75 & -11.65 & 22.84 & -5.29  & -0.76 & 4.89 & 33.71 & -4.79  & & & &  \\
     &  & -12.21 & -11.65 & 16.68 & -5.43  & & & &  & & & &  \\
     & 325 & 9.19 & -12.41 & 22.54 & -5.29  & -0.73 & 5.14 & 33.10 & -4.78  & & & &  \\
     &  & -12.48 & -12.41 & 16.80 & -5.42  & & & &  & & & &  \\
     & 350 & 9.57 & -12.16 & 22.38 & -5.30  & -0.56 & 5.64 & 32.37 & -4.78  & & & &  \\
     &  & -12.38 & -12.16 & 17.42 & -5.41  & & & &  & & & &  \\
    \hline
    80 & 0 & 27.14 & 11.90 & 9.85 & -6.69  & 0.12 & 7.64 & 37.01 & -4.78  & -0.28 & -9.40 & 41.03 & -4.83  \\
     &  & 12.09 & 11.90 & 21.29 & -5.37  & & & &  & & & &  \\
     &  & -12.73 & 11.90 & 22.39 & -5.35  & & & &  & & & &  \\
     & 25 & 11.94 & 10.65 & 23.95 & -5.33  & 0.26 & 5.89 & 36.97 & -4.78  & & & &  \\
     &  & -12.98 & 10.65 & 22.15 & -5.38  & & & &  & & & &  \\
     & 50 & 10.88 & 9.15 & 24.97 & -5.30  & 0.20 & 5.64 & 36.80 & -4.78  & & & &  \\
     &  & -13.40 & 9.15 & 20.86 & -5.42  & & & &  & & & &  \\
     & 75 & 10.81 & 10.15 & 24.07 & -5.30  & -0.03 & 7.14 & 38.10 & -4.79  & & & &  \\
     &  & -13.19 & 10.15 & 20.78 & -5.41  & & & &  & & & &  \\
     & 100 & 12.33 & 12.41 & 21.38 & -5.36  & -0.21 & -7.39 & 37.83 & -4.78  & & & &  \\
     &  & -12.02 & 12.41 & 22.70 & -5.35  & & & &  & & & &  \\
     & 125 & 15.99 & 14.41 & 9.42 & -6.34  & 8.56 & -9.40 & 24.61 & -5.02  & & & &  \\
     &  & 11.66 & 14.41 & 24.28 & -5.38  & -12.16 & -9.40 & 18.67 & -5.19  & & & &  \\
     &  & -12.74 & 14.41 & 22.39 & -5.37  & & & &  & & & &  \\
     & 150 & 13.63 & -12.41 & 21.96 & -5.37  & 8.12 & -9.65 & 25.13 & -5.00  & & & &  \\
     &  & -12.15 & -12.41 & 23.47 & -5.33  & -12.60 & -9.65 & 18.39 & -5.21  & & & &  \\
     & 175 & 12.85 & -12.66 & 23.77 & -5.35  & 10.14 & -8.65 & 23.07 & -5.08  & & & &  \\
     &  & -12.94 & -12.66 & 22.34 & -5.35  & -10.79 & -8.65 & 20.63 & -5.11  & & & &  \\
     & 200 & 12.28 & -11.65 & 24.56 & -5.34  & -0.56 & -5.64 & 37.47 & -4.78  & & & &  \\
     &  & -12.94 & -11.65 & 22.22 & -5.36  & & & &  & & & &  \\
     & 225 & 12.07 & -10.40 & 23.98 & -5.36  & -0.55 & -5.64 & 37.10 & -4.78  & & & &  \\
     &  & -12.34 & -10.40 & 22.64 & -5.35  & & & &  & & & &  \\
     & 250 & 11.90 & -10.15 & 23.22 & -5.37  & -0.36 & -6.64 & 37.30 & -4.78  & & & &  \\
     &  & -11.86 & -10.15 & 22.38 & -5.34  & & & &  & & & &  \\
     & 275 & 11.11 & -11.90 & 24.21 & -5.33  & -0.18 & 6.64 & 37.41 & -4.78  & & & &  \\
     &  & -12.58 & -11.90 & 20.58 & -5.38  & & & &  & & & &  \\
     & 300 & 10.71 & -13.66 & 24.79 & -5.30  & -0.14 & -7.89 & 37.63 & -4.78  & & & &  \\
     &  & -13.64 & -13.66 & 18.88 & -5.41  & & & &  & & & &  \\
     & 325 & 11.21 & -14.41 & 24.60 & -5.30  & -0.11 & -7.64 & 37.49 & -4.78  & & & &  \\
     &  & -13.95 & -14.41 & 19.74 & -5.41  & & & &  & & & &  \\
     & 350 & 11.78 & 12.16 & 23.85 & -5.31  & 0.04 & 7.89 & 37.01 & -4.78  & & & &  \\
     &  & -3.78 & 12.16 & 9.86 & -6.68  & & & &  & & & &  \\
     &  & -14.25 & 12.16 & 19.98 & -5.42  & & & &  & & & & 
\end{tabular}

==> tables/fits_sii-6730_1.tex <==
\begin{tabular}{ll|llll|llll|llll}
      &     & \multicolumn{4}{c}{MJ1} & \multicolumn{4}{c}{MJ5} & \multicolumn{4}{c}{REF} \\
    i[\degree] & phi [\degree] & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$)  \\
    \hline
    \hline
    0 & 0 & -4.08 & -4.39 & 10.91 & -5.86  & -3.58 & -3.88 & 10.61 & -5.92  & -3.98 & -3.88 & 10.22 & -5.58  \\
    \hline
    20 & 0 & -4.25 & -5.14 & 12.61 & -5.87  & -3.22 & -3.38 & 12.18 & -5.92  & -4.16 & -4.64 & 11.65 & -5.58  \\
     & 25 & -4.24 & -5.14 & 12.59 & -5.87  & -3.21 & -3.38 & 12.24 & -5.92  & & & &  \\
     & 50 & -4.25 & -5.14 & 12.66 & -5.87  & -3.26 & -3.63 & 12.45 & -5.92  & & & &  \\
     & 75 & -4.28 & -5.14 & 12.76 & -5.87  & -3.36 & -3.88 & 12.71 & -5.92  & & & &  \\
     & 100 & -4.34 & -5.14 & 12.81 & -5.87  & -3.48 & -3.88 & 12.90 & -5.92  & & & &  \\
     & 125 & -4.40 & -5.14 & 12.81 & -5.87  & -3.60 & -4.14 & 12.95 & -5.92  & & & &  \\
     & 150 & -4.43 & -5.14 & 12.76 & -5.87  & -3.74 & -4.39 & 12.83 & -5.92  & & & &  \\
     & 175 & -4.44 & -5.14 & 12.62 & -5.87  & -3.86 & -4.64 & 12.53 & -5.92  & & & &  \\
     & 200 & -4.41 & -4.89 & 12.43 & -5.87  & -3.89 & -4.39 & 12.17 & -5.93  & & & &  \\
     & 225 & -4.34 & -4.89 & 12.28 & -5.87  & -3.81 & -4.14 & 11.96 & -5.93  & & & &  \\
     & 250 & -4.27 & -4.64 & 12.28 & -5.87  & -3.66 & -3.88 & 11.99 & -5.93  & & & &  \\
     & 275 & -4.21 & -4.64 & 12.39 & -5.87  & -3.53 & -3.63 & 12.14 & -5.92  & & & &  \\
     & 300 & -4.20 & -4.89 & 12.53 & -5.87  & -3.43 & -3.38 & 12.28 & -5.92  & & & &  \\
     & 325 & -4.23 & -4.89 & 12.62 & -5.87  & -3.33 & -3.38 & 12.27 & -5.92  & & & &  \\
     & 350 & -4.24 & -4.89 & 12.62 & -5.87  & -3.25 & -3.38 & 12.20 & -5.92  & & & &  \\
    \hline
    40 & 0 & -3.82 & -6.14 & 17.64 & -5.87  & -2.26 & -1.63 & 16.46 & -5.92  & -3.63 & -5.14 & 16.48 & -5.58  \\
     & 25 & -3.72 & -5.64 & 17.83 & -5.87  & -2.22 & -1.63 & 16.12 & -5.92  & & & &  \\
     & 50 & -3.62 & -5.64 & 18.33 & -5.87  & -2.37 & -2.13 & 16.50 & -5.92  & & & &  \\
     & 75 & -3.64 & -5.89 & 18.49 & -5.87  & -2.63 & -2.88 & 17.36 & -5.92  & & & &  \\
     & 100 & -3.76 & -5.89 & 18.30 & -5.86  & -2.85 & -2.13 & 18.28 & -5.92  & & & &  \\
     & 125 & -3.85 & -5.64 & 18.16 & -5.87  & -3.03 & -1.38 & 18.64 & -5.92  & & & &  \\
     & 150 & -3.89 & -5.64 & 18.12 & -5.87  & -3.26 & -2.63 & 18.37 & -5.92  & & & &  \\
     & 175 & -3.92 & -5.89 & 17.93 & -5.87  & -3.54 & -4.39 & 16.84 & -5.92  & & & &  \\
     & 200 & -3.94 & -5.64 & 17.68 & -5.87  & -3.64 & -4.14 & 15.62 & -5.93  & & & &  \\
     & 225 & -3.89 & -4.39 & 17.48 & -5.87  & -3.43 & -3.38 & 15.16 & -5.93  & & & &  \\
     & 250 & -3.78 & -4.64 & 17.59 & -5.87  & -3.09 & -2.13 & 15.57 & -5.93  & & & &  \\
     & 275 & -3.72 & -5.14 & 17.74 & -5.87  & -2.86 & -1.38 & 16.56 & -5.92  & & & &  \\
     & 300 & -3.75 & -5.14 & 17.72 & -5.87  & -2.70 & -1.13 & 17.53 & -5.93  & & & &  \\
     & 325 & -3.83 & -5.64 & 17.73 & -5.86  & -2.53 & -0.88 & 17.58 & -5.93  & & & &  \\
     & 350 & -3.84 & -6.14 & 17.66 & -5.87  & -2.33 & -1.38 & 16.83 & -5.92  & & & &  \\
     \hline
    60 & 0 & -2.52 & -7.14 & 22.70 & -5.86  & -0.93 & 1.88 & 20.59 & -5.92  & -2.39 & -7.39 & 21.09 & -5.58  \\
     & 25 & -2.37 & -7.39 & 22.97 & -5.87  & -0.79 & 0.88 & 19.48 & -5.92  & & & &  \\
     & 50 & -2.25 & -7.64 & 23.38 & -5.87  & -1.04 & 0.38 & 20.01 & -5.92  & & & &  \\
     & 75 & -2.29 & -7.64 & 23.45 & -5.86  & -1.46 & -2.88 & 21.59 & -5.92  & & & &  \\
     & 100 & -2.43 & -7.39 & 23.29 & -5.86  & -1.77 & 2.63 & 23.17 & -5.93  & & & &  \\
     & 125 & -2.51 & -6.89 & 23.47 & -5.87  & -2.01 & 2.63 & 23.29 & -5.92  & & & &  \\
     & 150 & -2.53 & -7.14 & 23.53 & -5.87  & -2.30 & 1.63 & 23.35 & -5.92  & & & &  \\
     & 175 & -2.60 & -7.39 & 23.15 & -5.87  & -2.71 & -4.64 & 21.06 & -5.92  & & & &  \\
     & 200 & -2.67 & -7.64 & 22.75 & -5.87  & -2.95 & -4.14 & 18.91 & -5.93  & & & &  \\
     & 225 & -2.67 & -7.39 & 22.66 & -5.87  & -2.70 & -4.39 & 18.51 & -5.93  & & & &  \\
     & 250 & -2.58 & -7.64 & 22.96 & -5.87  & -2.21 & -0.13 & 19.87 & -5.93  & & & &  \\
     & 275 & -2.48 & -7.64 & 23.42 & -5.87  & -1.87 & 1.63 & 21.47 & -5.92  & & & &  \\
     & 300 & -2.48 & -6.89 & 23.68 & -5.87  & -1.67 & 3.38 & 22.73 & -5.92  & & & &  \\
     & 325 & -2.55 & -6.89 & 23.23 & -5.87  & -1.42 & 3.63 & 22.56 & -5.92  & & & &  \\
     & 350 & -2.56 & -7.14 & 22.73 & -5.86  & -1.07 & 2.63 & 21.32 & -5.92  & & & &  \\
\end{tabular}

==> tables/fits_sii-6730_2.tex <==
\begin{tabular}{ll|llll|llll|llll}
      &     & \multicolumn{4}{c}{MJ1} & \multicolumn{4}{c}{MJ5} & \multicolumn{4}{c}{REF} \\
    i[°] & phi [°] & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$) & v$_c$ & v$_p$ & FWHM & log(L/L$_\odot$)  \\
    \hline
    \hline
    80 & 0 & -0.77 & -6.39 & 25.53 & -5.86  & 0.52 & 4.14 & 22.69 & -5.92  & 5.40 & -6.89 & 12.81 & -5.87  \\
     &  & & & &  & & & &  & -7.52 & -6.89 & 11.42 & -5.92  \\
     & 25 & -0.62 & -6.64 & 25.67 & -5.87  & 0.74 & 3.38 & 21.11 & -5.93  & & & &  \\
     & 50 & -0.53 & 5.39 & 25.57 & -5.86  & 0.41 & 3.13 & 21.55 & -5.92  & & & &  \\
     & 75 & -0.59 & -7.14 & 25.79 & -5.86  & -0.12 & -3.13 & 23.58 & -5.93  & & & &  \\
     & 100 & -0.73 & -6.89 & 25.83 & -5.86  & -0.48 & -5.64 & 25.20 & -5.92  & & & &  \\
     & 125 & -0.78 & -6.14 & 26.44 & -5.86  & 5.82 & 5.39 & 11.16 & -6.43  & & & &  \\
     &  & & & &  & 0.28 & 5.39 & 28.37 & -6.34  & & & &  \\
     &  & & & &  & -8.34 & 5.39 & 11.13 & -6.43  & & & &  \\
     & 150 & -0.78 & 3.88 & 26.52 & -5.87  & 5.12 & -7.64 & 14.65 & -6.18  & & & &  \\
     &  & & & &  & -8.76 & -7.64 & 12.15 & -6.29  & & & &  \\
     & 175 & -0.85 & 4.39 & 25.99 & -5.87  & -1.54 & -5.39 & 23.37 & -5.92  & & & &  \\
     & 200 & -0.97 & -6.89 & 25.45 & -5.86  & -1.87 & -3.88 & 21.00 & -5.93  & & & &  \\
     & 225 & -1.04 & -6.89 & 25.13 & -5.86  & -1.62 & -4.64 & 20.71 & -5.93  & & & &  \\
     & 250 & -0.97 & -7.39 & 25.79 & -5.86  & -1.06 & 1.88 & 22.81 & -5.93  & & & &  \\
     & 275 & -0.85 & 5.14 & 25.95 & -5.86  & -0.66 & 4.14 & 24.36 & -5.92  & & & &  \\
     & 300 & -0.81 & 4.14 & 26.63 & -5.87  & 6.90 & -6.64 & 12.59 & -6.25  & & & &  \\
     &  & & & &  & -7.09 & -6.64 & 13.11 & -6.22  & & & &  \\
     & 325 & -0.83 & -5.89 & 26.34 & -5.87  & 7.61 & -6.39 & 9.62 & -6.58  & & & &  \\
     &  & & & &  & 0.44 & -6.39 & 29.24 & -6.40  & & & &  \\
     &  & & & &  & -2.29 & -6.39 & 19.37 & -6.47  & & & &  \\
     &  & & & &  & -7.39 & -6.39 & 9.42 & -6.68  & & & &  \\
     & 350 & -0.81 & -6.14 & 25.57 & -5.86  & 0.33 & 5.14 & 23.69 & -5.92  & & & & 
\end{tabular}
